The calculus of neo-Peircean relations

The calculus of relations was introduced by De Morgan and Peirce during the second half of the 19th century, as an extension of Boole's algebra of classes. Later developments on quantification theory by Frege and Peirce himself, paved the way to what is known today as first-order logic, causing the calculus of relations to be long forgotten. This was until 1941, when Tarski raised the question on the existence of a complete axiomatisation for it. This question found only negative answers: there is no finite axiomatisation for the calculus of relations and many of its fragments, as shown later by several no-go theorems. In this paper we show that -- by moving from traditional syntax (cartesian) to a diagrammatic one (monoidal) -- it is possible to have complete axiomatisations for the full calculus. The no-go theorems are circumvented by the fact that our calculus, named the calculus of neo-Peircean relations, is more expressive than the calculus of relations and, actually, as expressive as first-order logic. The axioms are obtained by combining two well known categorical structures: cartesian and linear bicategories.

==> tikz/proofs/henkinProp/tensorPlus.tex <==
% {\allowdisplaybreaks
% \[
%     \begin{array}{r@{\;}c@{\;}l}
%         &\HenFunctor(\scalebox{0.8}{\tensorCirc[+]{c}{d}})& \\[20pt]
%         &\Leq{\text{Def. }\HenFunctor}&  \HenFunctor(\scalebox{0.8}{\boxCirc[+]{c}}) \tensor[+] \HenFunctor(\scalebox{0.8}{\boxCirc[+]{d}}) \\[15pt]
%         &\Leq{\text{Ind. hyp.}}& \begin{aligned}
%             &\{ (\nterm{k_1},\nterm{l_1} \in X^n \times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_1}}{c}{\nterm{l_1}}} \} \\
%             \tensor[+] &\{ (\nterm{k_2},\nterm{l_2}) \in X^o \times X^p \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_2}}{d}{\nterm{l_2}}} \}
%         \end{aligned} \\[20pt]
%         &\Leq{\eqref{eq:tensorREL}}&    \begin{aligned}
%             \{ ( \Bigl( \begin{smallmatrix} \nterm{k_1} \\ \nterm{k_2} \end{smallmatrix} \Bigr), \Bigl( \begin{smallmatrix} \nterm{l_1} \\ \nterm{l_2} \end{smallmatrix} \Bigr) ) \in X^{n+o} \times X^{m+p} \mid &\scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_1}}{c}{\nterm{l_1}}} \\
%             \wedge &\scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_2}}{d}{\nterm{l_2}}} \}
%         \end{aligned} \\
%         &\Leq{\footnotesize{\stackanchor{\eqref{ax:comPlusLaxNat}}{\eqref{ax:discPlusLaxNat}}}}& \{ ( \Bigl( \begin{smallmatrix} \nterm{k_1} \\ \nterm{k_2} \end{smallmatrix} \Bigr), \Bigl( \begin{smallmatrix} \nterm{l_1} \\ \nterm{l_2} \end{smallmatrix} \Bigr) ) \in X^{n+o} \times X^{m+p} \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{{T}}} \scalebox{0.8}{\closedDecomposedTensorCirc{\nterm{k_1}}{\nterm{k_2}}{c}{d}{\nterm{l_1}}{\nterm{l_2}}} \} 
%         \\[20pt]
%         &\Leq{\text{Prop. }~\ref{prop:nary maps}}& \begin{aligned}
%             \{ (\nterm{k}, \nterm{l}) \in X^{n+o} \times X^{m+p} \mid &\scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedTensorCirc{k}{c}{d}{l}} \, , \\
%             &\qquad\nterm{k} = \nterm{k_1} \tensor[+] \nterm{k_2}, \nterm{l} = \nterm{l_1} \tensor[+] \nterm{l_2} \}
%         \end{aligned}      
%     \end{array}
% \]
% }
{\allowdisplaybreaks
    \begin{align*}
        &\HenFunctor(\scalebox{0.8}{\tensorCirc[+]{c}{d}}) \\
        &=  \HenFunctor(\scalebox{0.8}{\boxCirc[+]{c}}) \tensor[+] \HenFunctor(\scalebox{0.8}{\boxCirc[+]{d}}) \tag{\ref{fig:semantics}} \\
        &= \begin{array}{l}\{ (\nterm{k_1},\nterm{l_1}) \in X^n \times X^m \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_1}}{c}{\nterm{l_1}}} \} \tensor[+] \\ \{ (\nterm{k_2},\nterm{l_2}) \in X^o \times X^p \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_2}}{d}{\nterm{l_2}}} \} \end{array}\tag{Ind. hyp.} \\
        &=  \{ ( \Bigl( \begin{smallmatrix} \nterm{k_1} \\ \nterm{k_2} \end{smallmatrix} \Bigr), \Bigl( \begin{smallmatrix} \nterm{l_1} \\ \nterm{l_2} \end{smallmatrix} \Bigr) ) \in X^{n+o} \times X^{m+p} \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_1}}{c}{\nterm{l_1}}} \wedge \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedFormulaCirc{\nterm{k_2}}{d}{\nterm{l_2}}} \} \tag{\ref{eq:tensorREL}} \\
        &= \{ ( \Bigl( \begin{smallmatrix} \nterm{k_1} \\ \nterm{k_2} \end{smallmatrix} \Bigr), \Bigl( \begin{smallmatrix} \nterm{l_1} \\ \nterm{l_2} \end{smallmatrix} \Bigr) ) \in X^{n+o} \times X^{m+p} \mid \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{{T}}} \scalebox{0.8}{\closedDecomposedTensorCirc{\nterm{k_1}}{\nterm{k_2}}{c}{d}{\nterm{l_1}}{\nterm{l_2}}} \} \tag{\eqref{ax:comPlusLaxNat},\eqref{ax:discPlusLaxNat}} \\
        &= \{ (\nterm{k}, \nterm{l}) \in X^{n+o} \times X^{m+p} \!\mid\! \scalebox{0.8}{\emptyCirc[+]} \precongR{\T{T}} \scalebox{0.8}{\closedTensorCirc{k}{c}{d}{l}} , \nterm{k} = \nterm{k_1} \tensor[+] \nterm{k_2}, \nterm{l} = \nterm{l_1} \tensor[+] \nterm{l_2} \} \tag{Proposition~\ref{prop:nary maps}}
    \end{align*}
}

==> tikz/proofs/implication/capped.tex <==
\begin{align*}
    \cappedCirc[+]{b}
    &\Lleq{\footnotesize{\stackanchor{Lemma}{\ref{lm:id cup}}}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (109) at (-1.25, 0.25) {};
            \node [style=none] (122) at (-1.25, -1.125) {};
            \node [style=none] (123) at (-1.25, 1.05) {};
            \node [style=none] (124) at (3.375, 1.05) {};
            \node [style=none] (125) at (3.375, -1.125) {};
            \node [{dotStyle/-}] (128) at (2.125, -0.125) {};
            \node [style=none] (129) at (1.625, 0.25) {};
            \node [style=none] (130) at (1.625, -0.5) {};
            \node [{dotStyle/-}] (131) at (2.75, -0.125) {};
            \node [style=none] (133) at (-1.25, -0.5) {};
            \node [{boxStyle/+}] (134) at (-0.5, 0.25) {$b$};
            \node [style=none] (135) at (0.25, -0.875) {};
            \node [style=none] (136) at (0.25, 0.8) {};
            \node [style=none] (137) at (3.125, 0.8) {};
            \node [style=none] (138) at (3.125, -0.875) {};
            \node [style=none] (139) at (0.25, 0.25) {};
            \node [style=none] (140) at (0.625, 0.25) {};
            \node [style=none] (141) at (0.625, 0) {};
            \node [style=none] (142) at (0.625, 0.5) {};
            \node [style=none] (143) at (1.625, 0.5) {};
            \node [style=none] (144) at (1.625, 0) {};
            \node [style=none] (145) at (0.25, -0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/+}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{bgStyle/-}] (137.center)
                 to (136.center)
                 to (135.center)
                 to (138.center)
                 to cycle;
            \draw [{bgStyle/+}] (144.center)
                 to (143.center)
                 to (142.center)
                 to (141.center)
                 to cycle;
            \draw [{wStyle/-}, bend right] (130.center) to (128);
            \draw [{wStyle/-}, bend right] (128) to (129.center);
            \draw [{wStyle/-}] (128) to (131);
            \draw [{wStyle/+}] (109.center) to (134);
            \draw [style={wStyle/+}] (134) to (139.center);
            \draw [style={wStyle/-}] (139.center) to (140.center);
            \draw [style={wStyle/+}] (140.center) to (129.center);
            \draw [style={wStyle/+}] (145.center) to (133.center);
            \draw [style={wStyle/-}] (130.center) to (145.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \Lleq{\eqref{ax:leftLinDistr}} 
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (109) at (-1, 0.25) {};
            \node [style=none] (122) at (-1.25, -1.125) {};
            \node [style=none] (123) at (-1.25, 1.1) {};
            \node [style=none] (124) at (3.625, 1.1) {};
            \node [style=none] (125) at (3.625, -1.125) {};
            \node [{dotStyle/-}] (128) at (2.625, -0.125) {};
            \node [style=none] (129) at (2.125, 0.25) {};
            \node [style=none] (130) at (2.125, -0.5) {};
            \node [{dotStyle/-}] (131) at (3.25, -0.125) {};
            \node [style=none] (133) at (-1, -0.5) {};
            \node [{boxStyle/+}] (134) at (-0.25, 0.25) {$b$};
            \node [style=none] (135) at (-1, -0.875) {};
            \node [style=none] (136) at (-1, 0.85) {};
            \node [style=none] (137) at (2.125, 0.85) {};
            \node [style=none] (138) at (2.125, -0.875) {};
            \node [style=none] (139) at (0.5, 0.25) {};
            \node [style=none] (141) at (0.7, 0) {};
            \node [style=none] (142) at (0.7, 0.5) {};
            \node [style=none] (143) at (1.7, 0.5) {};
            \node [style=none] (144) at (1.7, 0) {};
            \node [style=none] (145) at (0.5, -0.5) {};
            \node [style=none] (146) at (0.5, -0.75) {};
            \node [style=none] (147) at (0.5, 0.725) {};
            \node [style=none] (148) at (1.875, 0.725) {};
            \node [style=none] (149) at (1.875, -0.75) {};
            \node [style=none] (150) at (1.875, 0.25) {};
            \node [style=none] (151) at (1.875, -0.5) {};
            \node [style=none] (152) at (1.7, 0.25) {};
            \node [style=none] (153) at (0.7, 0.25) {};
            \node [style=none] (154) at (-1.25, 0.25) {};
            \node [style=none] (155) at (-1.25, -0.5) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{bgStyle/+}] (137.center)
                 to (136.center)
                 to (135.center)
                 to (138.center)
                 to cycle;
            \draw [{bgStyle/-}] (149.center)
                 to (148.center)
                 to (147.center)
                 to (146.center)
                 to cycle;
            \draw [{bgStyle/+}] (144.center)
                 to (143.center)
                 to (142.center)
                 to (141.center)
                 to cycle;
            \draw [{wStyle/-}, bend right] (130.center) to (128);
            \draw [{wStyle/-}, bend right] (128) to (129.center);
            \draw [{wStyle/+}] (109.center) to (134);
            \draw [style={wStyle/+}] (134) to (139.center);
            \draw [style={wStyle/+}] (145.center) to (133.center);
            \draw [style={wStyle/-}] (139.center) to (153.center);
            \draw [style={wStyle/-}] (152.center) to (150.center);
            \draw [style={wStyle/+}] (129.center) to (150.center);
            \draw [style={wStyle/+}] (153.center) to (152.center);
            \draw [style={wStyle/-}] (151.center) to (145.center);
            \draw [style={wStyle/-}] (154.center) to (109.center);
            \draw [style={wStyle/-}] (155.center) to (133.center);
            \draw [style={wStyle/-}] (128) to (131);
            \draw [style={wStyle/+}] (151.center) to (130.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    \Lleq{\eqref{ax:linStrn4}}
    \begin{tikzpicture}
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (109) at (-0.9, 0.5) {};
            \node [style=none] (122) at (-1.25, -1.25) {};
            \node [style=none] (123) at (-1.25, 1.35) {};
            \node [style=none] (124) at (3.15, 1.35) {};
            \node [style=none] (125) at (3.15, -1.25) {};
            \node [{dotStyle/-}] (128) at (2.15, -0.075) {};
            \node [style=none] (129) at (1.475, 0.5) {};
            \node [style=none] (130) at (1.475, -0.625) {};
            \node [{dotStyle/-}] (131) at (2.775, -0.075) {};
            \node [style=none] (133) at (-0.9, -0.625) {};
            \node [{boxStyle/+}] (134) at (-0.25, 0.5) {$b$};
            \node [style=none] (141) at (-0.9, -0.1) {};
            \node [style=none] (142) at (-0.9, 1.1) {};
            \node [style=none] (143) at (1.2, 1.1) {};
            \node [style=none] (144) at (1.2, -0.1) {};
            \node [style=none] (151) at (1.2, -0.625) {};
            \node [style=none] (152) at (1.2, 0.5) {};
            \node [style=none] (154) at (-1.25, 0.5) {};
            \node [style=none] (155) at (-1.25, -0.625) {};
            \node [style=none] (156) at (-0.9, -1) {};
            \node [style=none] (157) at (-0.9, -0.275) {};
            \node [style=none] (158) at (1.2, -0.275) {};
            \node [style=none] (159) at (1.2, -1) {};
            \node [style=none] (160) at (0.15, -0.85) {};
            \node [style=none] (161) at (0.15, -0.425) {};
            \node [style=none] (162) at (1, -0.425) {};
            \node [style=none] (163) at (1, -0.85) {};
            \node [style=none] (164) at (0.15, -0.625) {};
            \node [style=none] (165) at (1, -0.625) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw [{bgStyle/-}] (124.center)
                 to (123.center)
                 to (122.center)
                 to (125.center)
                 to cycle;
            \draw [{bgStyle/+}] (144.center)
                 to (143.center)
                 to (142.center)
                 to (141.center)
                 to cycle;
            \draw [{bgStyle/+}] (159.center)
                 to (158.center)
                 to (157.center)
                 to (156.center)
                 to cycle;
            \draw [{bgStyle/-}] (163.center)
                 to (162.center)
                 to (161.center)
                 to (160.center)
                 to cycle;
            \draw [{wStyle/-}, bend right] (130.center) to (128);
            \draw [{wStyle/-}, bend right] (128) to (129.center);
            \draw [style={wStyle/-}] (154.center) to (109.center);
            \draw [style={wStyle/-}] (155.center) to (133.center);
            \draw [style={wStyle/-}] (128) to (131);
            \draw [style={wStyle/+}] (109.center) to (134);
            \draw [style={wStyle/+}] (134) to (152.center);
            \draw [style={wStyle/-}] (152.center) to (129.center);
            \draw [style={wStyle/-}] (151.center) to (130.center);
            \draw [style={wStyle/-}] (164.center) to (165.center);
            \draw [style={wStyle/+}] (165.center) to (151.center);
            \draw [style={wStyle/+}] (164.center) to (133.center);
        \end{pgfonlayer}
    \end{tikzpicture}                                           
    \structuralcong
    \cappedCirc[-]{b}     
\end{align*}
% \[
%     \circleCirc{\rla{b}}{b}
%     \Lgeq{b \Vdash \rla{b}}
%     \begin{tikzpicture}
%         \begin{pgfonlayer}{nodelayer}
%             \node [style=none] (122) at (2.125, -1) {};
%             \node [style=none] (123) at (2.125, 1) {};
%             \node [style=none] (124) at (-2.125, 1) {};
%             \node [style=none] (125) at (-2.125, -1) {};
%             \node [{dotStyle/-}] (128) at (-1.125, -0.125) {};
%             \node [style=none] (129) at (-0.5, 0.375) {};
%             \node [style=none] (130) at (-0.5, -0.625) {};
%             \node [{dotStyle/-}] (131) at (-1.75, -0.125) {};
%             \node [style=none] (133) at (0, -0.625) {};
%             \node [{dotStyle/-}] (135) at (1.125, -0.125) {};
%             \node [style=none] (136) at (0.5, 0.375) {};
%             \node [style=none] (137) at (0.5, -0.625) {};
%             \node [{dotStyle/-}] (138) at (1.75, -0.125) {};
%             \node [style=none] (139) at (0.5, 0.1) {};
%             \node [style=none] (140) at (0.5, 0.675) {};
%             \node [style=none] (141) at (-0.5, 0.675) {};
%             \node [style=none] (142) at (-0.5, 0.1) {};
%         \end{pgfonlayer}
%         \begin{pgfonlayer}{edgelayer}
%             \draw [{bgStyle/-}] (124.center)
%                  to (123.center)
%                  to (122.center)
%                  to (125.center)
%                  to cycle;
%             \draw [{bgStyle/+}] (141.center)
%                  to (140.center)
%                  to (139.center)
%                  to (142.center)
%                  to cycle;
%             \draw [{wStyle/-}, bend left] (130.center) to (128);
%             \draw [{wStyle/-}, bend left] (128) to (129.center);
%             \draw [{wStyle/-}] (128) to (131);
%             \draw [{wStyle/-}] (130.center) to (133.center);
%             \draw [{wStyle/-}, bend right] (137.center) to (135);
%             \draw [{wStyle/-}, bend right] (135) to (136.center);
%             \draw [{wStyle/-}] (135) to (138);
%             \draw [style={wStyle/-}] (133.center) to (137.center);
%             \draw [style={wStyle/+}] (129.center) to (136.center);
%         \end{pgfonlayer}
%     \end{tikzpicture}
%     \Lgeq{\text{Lemma }~\ref{lm:bool alg}}    
%     \begin{tikzpicture}
%         \begin{pgfonlayer}{nodelayer}
%             \node [style=none] (122) at (1.875, -1) {};
%             \node [style=none] (123) at (1.875, 1) {};
%             \node [style=none] (124) at (-1.875, 1) {};
%             \node [style=none] (125) at (-1.875, -1) {};
%             \node [{dotStyle/+}] (128) at (-0.375, 0) {};
%             \node [style=none] (129) at (-1, 0) {};
%             \node [{dotStyle/-}] (131) at (-1.5, 0) {};
%             \node [{dotStyle/+}] (135) at (0.375, 0) {};
%             \node [style=none] (136) at (1, 0) {};
%             \node [{dotStyle/-}] (138) at (1.5, 0) {};
%             \node [style=none] (139) at (1, -0.475) {};
%             \node [style=none] (140) at (1, 0.475) {};
%             \node [style=none] (141) at (-1, 0.475) {};
%             \node [style=none] (142) at (-1, -0.475) {};
%         \end{pgfonlayer}
%         \begin{pgfonlayer}{edgelayer}
%             \draw [{bgStyle/-}] (124.center)
%                  to (123.center)
%                  to (122.center)
%                  to (125.center)
%                  to cycle;
%             \draw [{bgStyle/+}] (141.center)
%                  to (140.center)
%                  to (139.center)
%                  to (142.center)
%                  to cycle;
%             \draw [style={wStyle/+}] (135) to (136.center);
%             \draw [style={wStyle/+}] (128) to (129.center);
%             \draw [style={wStyle/-}] (138) to (136.center);
%             \draw [style={wStyle/-}] (129.center) to (131);
%         \end{pgfonlayer}
%     \end{tikzpicture}
%     \Leq{\text{Prop. }~\ref{prop:maps}}
%     \begin{tikzpicture}
%         \begin{pgfonlayer}{nodelayer}
%             \node [style=none] (122) at (1.875, -1) {};
%             \node [style=none] (123) at (1.875, 1) {};
%             \node [style=none] (124) at (-1.875, 1) {};
%             \node [style=none] (125) at (-1.875, -1) {};
%             \node [{dotStyle/-}] (128) at (-0.875, 0) {};
%             \node [style={dotStyle/-}] (129) at (-1.5, 0) {};
%             \node [{dotStyle/-}] (135) at (0.875, 0) {};
%             \node [{dotStyle/-}] (138) at (1.5, 0) {};
%             \node [style=none] (139) at (0.5, -0.475) {};
%             \node [style=none] (140) at (0.5, 0.475) {};
%             \node [style=none] (141) at (-0.5, 0.475) {};
%             \node [style=none] (142) at (-0.5, -0.475) {};
%         \end{pgfonlayer}
%         \begin{pgfonlayer}{edgelayer}
%             \draw [{bgStyle/-}] (124.center)
%                  to (123.center)
%                  to (122.center)
%                  to (125.center)
%                  to cycle;
%             \draw [{bgStyle/+}] (141.center)
%                  to (140.center)
%                  to (139.center)
%                  to (142.center)
%                  to cycle;
%             \draw [style={wStyle/-}] (128) to (129);
%             \draw [style={wStyle/-}] (135) to (138);
%         \end{pgfonlayer}
%     \end{tikzpicture}    
%     \Lgeq{\eqref{ax:minusCodiscDisc}}
%     \emptyCirc[+]
% \]
